Beyond Gaussian Pyramid: Multi-skip Feature Stacking for Action Recognition

Most state-of-the-art action feature extractors involve differential operators, which act as highpass filters and tend to attenuate low frequency action information. This attenuation introduces bias to the resulting features and generates ill-conditioned feature matrices. The Gaussian Pyramid has been used as a feature enhancing technique that encodes scale-invariant characteristics into the feature space in an attempt to deal with this attenuation. However, at the core of the Gaussian Pyramid is a convolutional smoothing operation, which makes it incapable of generating new features at coarse scales. In order to address this problem, we propose a novel feature enhancing technique called Multi-skIp Feature Stacking (MIFS), which stacks features extracted using a family of differential filters parameterized with multiple time skips and encodes shift-invariance into the frequency space. MIFS compensates for information lost from using differential operators by recapturing information at coarse scales. This recaptured information allows us to match actions at different speeds and ranges of motion. We prove that MIFS enhances the learnability of differential-based features exponentially. The resulting feature matrices from MIFS have much smaller conditional numbers and variances than those from conventional methods. Experimental results show significantly improved performance on challenging action recognition and event detection tasks. Specifically, our method exceeds the state-of-the-arts on Hollywood2, UCF101 and UCF50 datasets and is comparable to state-of-the-arts on HMDB51 and Olympics Sports datasets. MIFS can also be used as a speedup strategy for feature extraction with minimal or no accuracy cost.

==> Experiments.tex <==

\section{Experiments}
We examine our hypothesis and the proposed MIFS representation on two tasks: action recognition and event detection. The experimental results show that MIFS representations outperforms conventional original-scale representations on five real-world challenging datasets. 

Improved Dense Trajectory with Fisher Vector encoding \cite{wang2013action} represents the current state-of-the-arts for most real-world action recognition datasets. Therefore, we use it to evaluate our method. Note that although we use Improved Dense Trajectory, our methods can be applied to any local features that using differential filters, e.g., STIP \cite{laptev2005space}. 


\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
                \includegraphics[width=\textwidth]{img/k1.pdf}
                \caption{HMDB51}
                \label{fig:lhmdb}
        \end{subfigure}%
~
        \begin{subfigure}[b]{0.3\textwidth}
                \includegraphics[width=\textwidth]{img/k2.pdf}
                \caption{Hollywood2}
                \label{afig:h2}
        \end{subfigure}
~                
        \begin{subfigure}[b]{0.3\textwidth}
                \includegraphics[width=\textwidth]{img/k3.pdf}
                \caption{UCF101}
                \label{fig:ucf101}
        \end{subfigure}
        \caption{The decaying trend of singular values of feature matrices for HMDB51,  Hollywood and UCF101 Datasets. 0 to 5 indicate the MIFS level and $i$ indicates the $i$th singular value. From all three datasets, we can see that MIFS representations do have a slower singular value decaying trend compared to conventional representations ({\color[rgb]{0,0,1} blue} lines). }\label{fig:trend}
\end{figure*}

\subsection{Action Recognition}
\label{action_recognition}
\paragraph{Problem Formulation}
The goal of this task is to recognize human actions in short clips of videos. 
\paragraph{Datasets}Three representative datasets are used: The HMDB51 dataset \cite{kuehne2011hmdb} has 51 action classes and 6766 video clips extracted from digitized movies and YouTube. \cite{kuehne2011hmdb} provides both original videos and stabilized ones. We only use original videos in this paper and standard splits with MAcc (mean accuracy) are used to evaluate the performance. The Hollywood2 dataset \cite{marszalek2009actions} contains 12 action classes and 1707 video clips that are collected from 69 different Hollywood movies. We use the standard splits with training and test videos provided by \cite{marszalek2009actions}.   Mean average precision (MAP) is used to evaluate this dataset because multiple labels can be assigned to one video clip. The UCF101 dataset \cite{soomro2012ucf101} has 101 action classes spanning over 13320 YouTube videos clips. We use the standard splits with training and test videos provided by \cite{soomro2012ucf101} and MAcc is reported.
\paragraph{Experimental setting}
Improved Dense Trajectory features are extracted using 15 frame tracking, camera motion stabilization and RootSIFT normalization and described by Trajectory, HOG, HOF, MBHx and MBHy descriptors. We use PCA to reduce the dimensionality of these descriptors by a factor of two. After reduction, we augmented the descriptors with three dimensional normalized  location information. The only difference between MIFS and other conventional methods is that instead of using feature points extracted from one time scale, we extract and stack all the raw feature points from different scales together before encoding. For Fisher Vector encoding,  we map the raw descriptors into a  Gaussian Mixture Model with 256 Gaussians trained from a set of randomly sampled 256000 data points. Power and L2 normalization are also used before concatenating different types of descriptors into a video based representation. For classification, we use a linear SVM classifier with a fixed $C=100$ as recommended by \cite{wang2013action} and the one-versus-all approach is used for multi-class classification scenario. 

\paragraph{Results}\hspace{0pt}

We first examine if it is true that the conditional number $\beta(PP^{\mathrm{T}})$ is improved by MIFS. However, it would not be meaningful to compute $\beta(PP^{\mathrm{T}})$ directly because we have noise
$\boldsymbol{\epsilon}$ in $\mathcal{F}[X(t),\tau_i]$ and the smallest singular value $\lambda_{min}$ is in noise space . A workaround is to examine the decaying speed of singular values of the feature matrix. The
singular values are normalized by dividing the maximum singlular value $\lambda_{\max}$.
We only plot the top $10$ singular values, since the subspace spanned by the
small singular values is noise space. Clearly, when MIFS improves the
learnability, we should get a slower decaying curve of the top $k$ singular
values. Shown in Figure \ref{fig:trend} are the trends of
$\frac{\lambda_i}{\lambda_{max}}$. On all three datasets, the singular values of MIFS decrease slower than the conventional one (0). It is also interesting to see  that by having one or two additional levels, we have already exploited most of the potential improvement.


We further examine how performance change with respect to the MIFS level, as shown in Table \ref{tab:scalePyramid}. First, let us compare the performance of L=0 to the standard location-insentative feature representation. Our performance on HMDB51, Hollywood2 and UCF101 datasets are $62.1\%$ MAcc, $67.0\%$ MAP and $87.3\%$ MAcc respectively. These numbers are higher than Wang \& Schmid \cite{wang2013action}'s results, which are $57.2\%$, $64.3\%$ and $85.9\%$, respectively. This is largely because of our location sensitive feature representation. Next, let us check the behavior of MIFS. For completeness, we list both single-scale and stacking performance. For single-scale performance, we observe that for HMDB51, its performance increases from $62.1\%$ to $63.1\%$ and then decrease rapidly, similar pattern can be seen in Hoollywood2 and UCF101 except their performance do not increase at $L=1$. These results consist with our observation that different actions need different scale ranges. They also substantiates our proof that selecting time interval $\tau$ is a trade-off between the feature bias and its variance. Now let us compare MIFS with single-scale representation. We observe that for MIFS representations, although there is still a bias and variance trade-off as in single-scale representations for different levels, they all perform better than single-scale representation and the performance decreasing points are later than those in the single-scale representations. We also observe that for MIFS representations, most of the performance improvement comes from $L=1$ and $L=2$, which supports what we observed in Figure \ref{fig:trend} that, in practice, having one or two more scales is enough to recover most of lost information due to the differential operations. Higher scale features become less reliable due to the increasing difficulty in optical flow estimation and tracking.  It is also interesting to observe that HMDB51 enjoys a higher performance improvement from MIFS than the Hollywood2 and UCF101 dataset has. We believe that one of the main reason is that HMDB dataset is a mixture of videos from two sources: Youtube and movie, which results in larger action velocity range than pure movie videos or Youtube in the other two datasets.

 


\begin{table*}
\centering
\begin{tabular}{|c | c |c |c |c |c| c| }
\hline
  & \multicolumn{2}{|c|}{HMDB51  (MAcc$\%$) } & \multicolumn{2}{|c|}{ Hollywood2 (MAP$\%$)} &\multicolumn{2}{|c|}{UCF101(MAcc$\%$)}   \\\hline
  L& Single-scale & MIFS & Single-scale & MIFS & Single-scale & MIFS\\\hline 

 0 &   62.1 &                   & 67.0 &                & 87.3 & \\
 1 &   63.1 & 63.8              & 66.4 & 67.5           & 87.3& 88.1\\
 2 &   54.3 & 64.4              & 62.5 & 67.9           & 85.5& 88.8\\
 3 &   43.8 & 65.1              & 60.5 & \textbf{68.0}  & 81.3& \textbf{89.1}\\
 4 &   24.1 & \textbf{65.4}     & 58.1 & 67.4           & 74.6& \textbf{89.1}\\
 5 &   15.9 & \textbf{65.4}     & 54.4 & 67.1           & 66.7& 89.0\\
\hline
\end{tabular}
\caption{\label{tab:scalePyramid}Comparison of different scale levels for MIFS.}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{|c c |c c |c c|}
\hline
    \multicolumn{2}{|c|}{HMDB51 (MAcc. $\%$)} & \multicolumn{2}{|c|}{Hollywood2 (MAP $\%$)} & \multicolumn{2}{|c|}{UCF101(MAcc. $\%$)}\\ \hline
    
Oneata \textit{et al.} \cite{oneata2013action} 13 &54.8 &  Lin \textit{et al.} \cite{sun2014dl} 14 & 48.1      &  Karpathy \textit{et al.} \cite{karpathy2014large} 14 & 65.4\\
Wang \& Schmid \cite{wang2013action} 13  &57.2   & Sapienz \textit{et al.} \cite{sapienza2014feature} 14 & 59.6   & Sapienz \textit{et al.} \cite{sapienza2014feature} 14 & 82.3\\
Simonyan \& Zisserman \cite{simonyan2014two} 14 & 57.9 &Jain \textit{et al.} \cite{jain2013better} 13   & 62.5  & Wang \& Schmid \cite{wang2013lear} 13 & 85.9 \\
Peng \textit{et al.} \cite{peng2014bag} 14 & 61.1  &  Oneata \textit{et al.} \cite{oneata2013action} 13&  63.3   &Simonyan \& Zisserman \cite{simonyan2014two} 14  & 87.6 \\
Peng \textit{et al.} \cite{peng2014bag} 14 & \textbf{66.79} & Wang \& Schmid \cite{wang2013action} 13 &64.3  &Peng \textit{et al.} \cite{peng2014bag} 14 &  87.9\\
\hline 
MIFS (L=3)  & 65.1 & MIFS (L = 3) &  \textbf{68.0} & MIFS (L = 3) & \textbf{89.1}\\ 
\hline
\end{tabular}
\caption{\label{tab:state-of-art}Comparison of our results to the state-of-the-arts.}
\end{table*}

\paragraph{Comparing with the State-of-the-Arts}
In Table \ref{tab:state-of-art}, we  compare MIFS at $L=3$, which perform well across all three action datasets, with the state-of-the-art approaches. From Table \ref{tab:state-of-art}, in all three datasets, we observe substantial improvement over the state-of-the-arts. Note that although we list several most recent approaches here for comparison purposes, \textit{most of them are not directly comparable to our results due to the use of of different features and representations}. The most comparable one is Wang \& Schmid. \cite{wang2013action}, from which we build on our approaches. Shao et al. \cite{zhen2013spatio} proposed to use Laplacian pyramid and Garbor filters to encode videos and get $37.3 \%$ accuracy on the HMDB51 dataset. Sapienz \textit{et al.} \cite{sapienza2014feature} explored ways to sub-sample and generate vocabularies for Dense Trajectory features. 
Jain et al. \cite{jain2013better}'s approach incorporated  a new motion descriptor. Oneata et al.  \cite{oneata2013action} focused on testing Spatial Fisher Vector for multiple action and event tasks. Peng et al. \cite{peng2014bag}  improved the performance of Improved Dense Trajectory by increasing the codebook size and fusing multiple coding methods. Karpathy et al. \cite{karpathy2014large} trained a deep convolutional neural network using 1 million weakly labeled YouTube videos and reported  65.4\% mean accuracy on UCF101 datasets. Simonyan \& Zisserman \cite{simonyan2014two} reported results that is competitive to Improved Dense Trajectory method by training deep convolutional neural networks using both sampled frames and optical flows and get $57.9\%$ MAcc in HMDB51 and $87.6\%$ MAcc in UCF101, which are comparable to the results of Wang $\&$ Schmid. 



\subsection{Event Detection}
\paragraph{Problem Formulation}
Given a collection of videos, the goal of an event detection task is to detect events of interest such as \textit{Birthday Party} and \textit{Parade}, solely based on the video content. The task is very challenging due to complex actions and scenes. Through this task, we examine whether MIFS can improve the performance of recognizing very complex actions. 

\paragraph{Dataset}
TREC Video Retrieval Evaluation (TRECVID) Multimedia Event Detection (MED) is a task organized by NIST (National Institute of Standards and Technology) aiming at encouraging new technologies for detecting complex events such as \textit{having a birthday party}. Started at 2010, NIST has gradually built up a database that contains 8000 hours of videos and 40 events, which is by far the largest event detection collection. MEDTEST13,14 datasets are two standard system evaluation datasets released by NIST in 2013 and 2014, respectively. Each of them contains around 10 percents of the whole MED collection and has 20 events. They consist of two tasks, i.e. EK100 and EK10. As their names suggest, EK100 task has 100 positive training samples while EK10 has 10. For both tasks, they have around 5000 background samples. Together, each dataset has 8000 training samples and 24000 testing samples. 

\paragraph{Experimental setting}A similar setting discussed in section \ref{action_recognition} is applied except we only test MIFS with L=3 as recommended in section \ref{action_recognition}. We do not test all the stacking levels in MEDTEST13,14 datasets because extracting Dense Trajectory feature from such large datasets itself is very time consuming. It took us 4 days to generate representations for both MEDTEST13,14 using a cluster with more than 500 Intel E565+ series processors. We use cross-validation to choose penalty parameter C for the linear SVM and MAP as evaluation criteria. 


\paragraph{Results} Table \ref{tab:med} lists the overall MAP. The baseline method is a conventional single-scale representation with $L=0$. From Table \ref{tab:med}, we can see that for both MEDTEST13 and MEDTEST14, MIFS representations consistently improve over the original-scale representation by about $2\%$ in both EK100 and EK10. It is worth emphasizing that MED is such a challenging task that $2\%$ of absolute performance improvement is quite significant. 


\begin{table}
\centering
\begin{tabular}{|c | c c|c c|}
\hline
 & \multicolumn{2}{|c|}{MEDTEST13}  & \multicolumn{2}{|c|}{MEDTEST14}\\
\hline 
 & EK100& EK10  & EK100 & EK10 \\\hline
  Baseline & 34.2 & 17.7& 12.7 & 27.3  \\ 
  MIFS (L=3) & \textbf{36.3}& \textbf{19.3} & \textbf{14.9} & \textbf{29.0}  \\
\hline
\end{tabular}
\caption{\label{tab:med}Performance Comparison on the MED task.}
\end{table}




\subsection{Computational Complexity}
Level 0 of a MIFS representation has the same cost as other single pass methods, e.g., Wang \& Schmid. \cite{wang2013action}.  For level $l$, the cost becomes $1/l$ of the level 0. So with a MIFS up to level 2, the computational cost will be less than twice the cost of a single pass through the original video, yet it can significantly improve the single-pass methods.

==> Introduction.tex <==
\section{Introduction}

We consider the problem of enhancing video representations for action recognition, which becomes increasingly important for both analyzing human activity itself and as a component for more complex event analysis. As pointed out by Marr \cite{marr1982vision} and Lindeberg \cite{lindeberg1994scale}, visual representations, or visual features, are of utmost importance for a vision system, not only because they are the chief reasons for tremendous progress in the field, but also because they lead to a deeper understanding of the information processing in the human vision system. In fact, most of the qualitative improvements to visual analysis can be attributed to the introduction of improved representations, from SIFT \cite{lowe2004distinctive} to to Deep Convolutional Neural Networks \cite{sermanet2013overfeat}, from STIP \cite{laptev2005space} to Dense Trajectory \cite{wang2011action} . A common characteristic of these several generations of visual features is that they all, in some way, benefit from the idea of multi-scale representation, which is generally viewed as an indiscriminately applicable tool that reliably yields an improvement in performance when applied to almost all feature extractors. 


\begin{figure}
        \centering
        \begin{subfigure}[b]{0.23\textwidth}
                \includegraphics[width=\textwidth]{img/kr_ma.jpg}
                \caption{Kids Running}
                \label{fig:kr}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.23\textwidth}
                \includegraphics[width=\textwidth]{img/or.jpg}
                \caption{Olympics Running}
                \label{fig:or}
        \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.22\textwidth}
                \includegraphics[width=\textwidth]{img/signal.pdf}
                \caption{Action signal $S$}
                \label{fig:signal}
        \end{subfigure}
       ~ \quad
        \begin{subfigure}[b]{0.22\textwidth}
                \includegraphics[width=\textwidth]{img/dsignal.pdf}
                \caption{  $\Delta S$ }
                \label{fig:dsignal}
        \end{subfigure}
        \caption{Simplified action signals (\ref{fig:signal}) from "running" actions (\ref{fig:kr},\ref{fig:or}) show dramatically difference among subjects and scenes. With such dramatic differences among action signals, a differential operator with single scale is incapable of covering a full range of action frequency and tend to lose low frequency information (the {\color[rgb]{1,0,0} red} and {\color[rgb]{0,0.44,0.75} cyan} signals) .  }\label{fig:motivation}
\end{figure}

At the core of image multi-scale representation is the requirement that no new detail information should be artificially found at the coarse scale of resolution \cite{koenderink1984structure}. Gaussian Pyramid, a unique solution based on this constraint, generates a family of images where fine-scale information is successively suppressed by Gaussian smoothing.  However, in action recognition, we often desire the opposite requirements.  For example, in generating action features using differential filters, we need coarse-scale  features to:  1) recover the information that has been filtered out by highpass filters at fine scales, e.g., the {\color[rgb]{1,0,0} red} and {\color[rgb]{0,0.44,0.75} cyan} signals in Figure \ref{fig:signal} are likely to be filtered out; 2) generate features at higher frequency for matching similar actions at different speeds and ranges of motion, e.g., the {\color[rgb]{1,0.75,0} orange} and {\color[rgb]{0,0.69,0.31} green} signals in Figure \ref{fig:signal}. Both of these requirements can not be satisfied with a Gaussian Pyramid representation. 


In this work, we introduce a Multi-skIp Feature Stacking (MIFS) representation that works by stacking features extracted by a family of differential filters parameterized with multiple time skips (scales). Our algorithm relies on the idea that by gradually reducing the frame rate, feature extractors with differential filters can extract information about more subtle movements of actions. MIFS has several attractive properties:
\begin{itemize}
\item Like Gaussian Pyramid, it is an indiscriminately applicable tool that can be reliably and easily adopted by any feature extractors with differential filters. 
\item It generates features that are shift-invariance in frequency space, hence easier to match similar actions at different speeds and ranges of motion. 
\item Compared to conventional action representations, it stacks features at multiple frequencies and tends to cover a longer range of action signals. 
\item Our theoretical analysis shows that it generates feature matrices that have lower conditional numbers and variances hence higher learnability compared to the conventional original-scale representation. 
\item Experimental results on several real-world benchmark datasets show that it significantly improves the performance of state-of-the-art methods.
\item MIFS exponentially enhances the learnability of the resulting feature matrices. Therefore the required additional number of scales is logarithmic to the bandwidth of the action signals. Empirical studies show that one or two additional scales are enough to recover the lost information lost. Hence the additional computational cost of MIFS is small.
\end{itemize}

In the remainder of this paper, we start by providing more background information about action recognition and multi-scale presentations. We then describe MIFS in detail, followed by theoretically proving that MIFS improves the learnability of video representations exponentially. After that, an evaluation of our method is performed. Further discussions including potential improvements are given at the end. 




==> Related_work.tex <==

\section{Related Work}
There is an extensive body of literature about action recognition; here we just mention a few relevant ones involved with state-of-the-art feature extractors and feature encoding methods. See \cite{aggarwal2011human} for an in-depth survey. In conventional video representations, features and encoding methods are the two chief reasons for considerable progress in the field. Among them, the trajectory based approaches \cite{matikainen2009trajectons,sun2009hierarchical,wang2011action,wang2013action,jiang2012trajectory}, especially the Dense Trajectory method proposed by Wang et al. \cite{wang2011action,wang2013action}, together with the Fisher Vector encoding  \cite{perronnin2010improving}  yields the current state-of-the-art performances on several benchmark action recognition datasets.  Peng et al. \cite{peng2014bag} further improved the performance of Dense Trajectory by increasing the codebook sizes and fusing multiple coding methods. Some success has been reported recently using deep convolutional neural networks for action recognition in videos. Karpathy et al. \cite{karpathy2014large} trained a deep convolutional neural network using 1 million weakly labeled YouTube videos and reported a moderate success on using it as a feature extractor. Simonyan $\&$ Zisserman \cite{simonyan2014two} reported a result that is competitive to Improved Dense Trajectory \cite{wang2013action} by training deep convolutional neural networks using both sampled frames and optical flows. MIFS is an indiscriminately applicable tool that can be adopted by all of above mentioned feature extractors. 

Multi-scale representation \cite{adelson1984pyramid, lindeberg1994linear} have been very popular for most image processing tasks such as image compression, image enhancement and object recognition. A multi-scale key-point detector proposed by Lindeberg \cite{lindeberg1993detecting} and used in by Lowe \cite{lowe2004distinctive} to detect scale invariant key points using Laplacian pyramid methods, in which Gaussian smoothing is used iteratively for each pyramid level. Simonyan $\&$ Zisserman \cite{simonyan2014very} reported a significant performance improvement on Imagenet Challenge 2014 by using a multi-scale deep convolutional neural network. In video processing, Space Time Interest Points (STIP) \cite{laptev2005space} extends SIFT to the temporal domain by finding the scale invariant feature points in 3D space. Shao et al. \cite{zhen2013spatio} also try to achieve scale invariance for action recognition using 3-D Laplacian pyramids and 3D Gabor filters. However, without awareness of the fundamental difference between image and video processing, \cite{zhen2013spatio} was not very successful when compared to the state-of-the-art methods. 


For lab datasets where human poses or action templates can be reliably estimated, Dynamic Time Warping (DTP) \cite{ darrell1993space}, Hidden Markov Models (HMMs) \cite{yamato1992recognizing, natarajan2007coupled} and Dynamic Bayesian Networks (DBNs) \cite{park2004hierarchical} are well studied methods for aligning actions that have speed variation. However, for noisy real-world actions, these methods have not shown themselves to be very robust. 



==> Video_Pyramids.tex <==

\section{ Multi-skIp Feature Stacking (MIFS)}


\begin{figure*}                   
        \begin{subfigure}[b]{0.43\textwidth}
                \includegraphics[width=\textwidth]{img/gp.pdf}
                \caption{ Gaussian Pyramid}
                \label{fig:gp}
        \end{subfigure}
       ~ \quad
        \begin{subfigure}[b]{0.43\textwidth}
                \includegraphics[width=\textwidth]{img/vp.pdf}
                \caption{  MIFS}
                \label{fig:mifs}
        \end{subfigure}
\caption{Comparison of Gaussian Pyramid and MIFS for the {\color[rgb]{1,0,0} red} signal in Figure \ref{fig:motivation}.The left figure (\ref{fig:gp}) shows that as the level ($L$) goes higher (from 1 to 3), the resulting features ($\Delta S$) from a differential operator become less prominent. So once a feature has been filtered out (assume the threshold for a feature to be represented is 0.1), it cannot be recovered by higher level features under the Gaussian Pyramid framework. The right figure (\ref{fig:mifs}) shows that under MIFS, the features ($\Delta S$) become more prominent as the levels go higher and can represent those signals that have been filtered out at low levels.}\label{fig:msr}
\end{figure*}


We now formalize our notation. For the present discussion a video $X$ is just a real function of three variables:
\begin{align}
X = X(x, y, t).
\end{align}
The normalized coordinates $(x, y, t) \in R^3$ are the  Cartesian coordinates
of the video space.
Since we focus on temporal domain, we omit $(x,y)$ in further discussion and
denote a video as $X(t)$. The length of the video is assumed to be normalized,
that is $t\in[0,1]$.
In our model, the content of a video is generated by a linear mixture of  $k$ latent signals:
\begin{align} \label{eq:video-latent-signal-model}
  \bar{X}=[\bar{\mathbf{x}}_{1},\bar{\mathbf{x}}_{2},\cdots,\bar{\mathbf{x}}_{k}] \ .
\end{align}


The mixing weight of each latent action signal
$\bar{\mathbf{x}}_{i}$ at time $t$ is denoted as $\alpha_{i}(t)$. Therefore, a
given video is generated as
\begin{align}
  X(t)=&\bar{X}\boldsymbol{\alpha}(t)+\boldsymbol{\epsilon}(t) \\
  \boldsymbol{\alpha}(t)=&[\alpha_{1}(t),\alpha_{2}(t),\cdots,\alpha_{k}(t)]{}^{\mathrm{T}}~.
\end{align}
where $\boldsymbol{\epsilon}(t)$ is additive subgaussian noise with noise level
$\sigma$. Without loss of generality, we assume $\forall i $,
\begin{align}
|\alpha_{i}(t)|\leq 1 & \quad  \mathrm{E}_{t}\{\alpha_{i}(t)\}=0 \\
\mathrm{E}_{t}\{\alpha_{i}(t)^{2}\}\leq1 &\quad  \mathrm{E}_{t}\{ \alpha_{i}(t) \times \alpha_{j}(t)|_{i\neq j}\} = 0   ~.
\end{align}


The feature extractor is assumed to be modeled as a differential operator
$\mathcal{F}[\cdot,\tau]$ parameterized with time skip $\tau$. Given a fixed
$\tau$, the feature extractor $\mathcal{F}[X(t),\tau]$ randomly generates $T
= \left\lfloor 1/\tau\right\rfloor $ features.
\[
\mathcal{F}[X(t),\tau]=[\mathbf{f}(t_{1},\tau),\mathbf{f}(t_{2},\tau),\cdots,\mathbf{f}(t_{T},\tau)]~.
\]
where $t_{1},t_{2},\cdots,t_{T}$ are uniformly sampled on $[0,1]$.
The $i$-th feature vector $\mathbf{f}(t_{i},\tau)$  is generated by
\begin{align}
f(t_{i},\tau) & = X(t_i+\tau)-X(t_i) \\
& =  \bar{X}\times(\boldsymbol{\alpha}(t_i+\tau)-\boldsymbol{\alpha}(t_i))+\boldsymbol{\epsilon}(t_i+\tau)-\boldsymbol{\epsilon}(t_i)~. \nonumber
\end{align}

We can rewrite the feature matrix  as
\[
\mathcal{F}[X(t),\tau]=\bar{X}P+\sum_{i=1}^{T}\boldsymbol{\epsilon}(t_{i}+\tau)-\boldsymbol{\epsilon}(t_{i})
\]
 where $P$ is a $k\times T$ matrix, $P_{i,j}=\boldsymbol{\alpha}_{i}(t_{j}+\tau)-\boldsymbol{\alpha}_{i}(t_j)$.
 
Most action feature extractors are different versions of $\mathcal{F}$. For
example, STIP \cite{laptev2005space} and Dense Trajectory
\cite{wang2011action} can be derived from $\mathcal{F}[\cdot, \frac{1}{L}]$,
where $L$ is the number of frames in the video.

MIFS stacks multiple $\mathcal{F}[X(t),\tau]$ with different $\tau$. By stacking multiple features with different frequencies, MIFS seeks invariance in the frequency domain via
resampling in the time domain. Figure \ref{fig:msr} shows the difference of Gaussian
Pyramid and MIFS for the {\color[rgb]{1,0,0} red} signal in Figure \ref{fig:motivation}. It is
clear that, because of smoothing, Gaussian Pyramid fails to recover signals once they have been filtered out. As the levels go higher, the feature generated by Gaussian Pyramids can only become weaker. While in MIFS, the generated features become more prominent and can be recovered as the levels go higher. 

\section{The Learnability of MIFS}


In this section, we first show that under model
Eq.~\eqref{eq:video-latent-signal-model}, the standard feature extraction
method cannot produce a  feature matrix conditioned well enough. Then we show that MIFS improves the condition number of the extracted feature matrix
exponentially. One of the key novelties of the MIFS is that it
also reduces the uncertainty of the feature matrix simultaneously. This reduction is not
possible in a naive approach.


\subsection{Condition Number of $P$ under a Fixed $\tau$}


In this subsection, we will prove, based on Bernstein's Matrix Inequality
\cite{tropp2012user},  that
the condition number of $P$ is not necessarily a small number. 

In static feature extractors  such as SIFT, the weight coefficient
matrix $\boldsymbol{\alpha}$ is independent of $t$. While in a video stream, the
action signal is dynamic in $t$. To measure the dynamic of an action signal, we introduce $\gamma_{i}$ as an
index.
\begin{defn}
\label{def:alpha-independent}A latent action signal is $\gamma$
dynamic, if given a positive constant $c\in(0,1)$, $\forall\tau\in[0,1]$,
\[
\ 1-(1+c)\exp(-\gamma/\tau)\leq\mathrm{E}_{t}|\alpha(t)\alpha(t+\tau)|\leq1-\exp(-\gamma/\tau)~,
\]
\end{defn}
The value $\gamma$ measures how fast the coefficient $\alpha(t)$ varies along
time $t$. Here we take the exponential function by assuming the correlation
between $\alpha(t+\tau)$ and $\alpha(t)$ to be at least subgaussian. If in a
given video, the $i$-th action signal is a high frequency component, then its
coefficient $\boldsymbol{\alpha}_{i}(t)$ will behave like a random number for 
time skip $\tau$. Therefore, we would expect that the correlation between
$\boldsymbol{\alpha}_{i}(t)$ and $\boldsymbol{\alpha}_{i}(t+\tau)$ is close to
0. Or if the action signal is a low frequency component, the correlation indicator $\gamma$ should
be close to $1$. For the sake of simplicity, we rearrange latent action
signal $\bar{X}$ by their frequency to have
$\gamma_{1}\leq\gamma_{2}\leq\cdots\leq\gamma_{k}$.


 In a learning problem, we hope the feature matrix $\mathcal{F}[X(t),\tau]$ is
 well conditioned. Given feature matrix $\mathcal{F}[X(t),\tau]$, we can
 recover $\bar{X}$ by various methods, such as subspace clustering. The
 sampling complexity of any recovery algorithm depends on the condition number
 of $P$. Clearly when $P$ is ill--conditioned, we require a large number of
 training examples to estimate $\bar{X}$. The learnability of
 $\mathcal{F}[X(t),\tau]$ depends on its condition number which in return
 depends on $P$ again. In the following, we will prove that for a fixed time
 skip $\tau$, $P$ is not necessarily well conditioned. Therefore the learnability of $\mathcal{F}[X(t),\tau]$ is suboptimal.The intuition
behind our proof is that when an action signal has a large $\gamma$, then a
small time skip $\tau$ will make the coefficient of that signal close to
zero. Therefore, $P$ is ill-conditioned.
Formally, we have the following
theorem to bound the condition number  $\beta(PP{}^{\mathrm{T}})$ of $PP{}^{\mathrm{T}}$(see the proof in supplementary materials). 

\begin{thm}
\label{thm:condition-number-P-under-fixed-tao} Given a fixed time
skip $\tau$, with probability at least $1-\delta$, the condition number
$\beta(PP{}^{\mathrm{T}})$ is bounded by
\begin{align}
  &\beta(PP{}^{\mathrm{T}})\leq\frac{(1+c)\exp(-\gamma_{1}/\tau)+\Delta_{\tau}}{\exp(-\gamma_{k}/\tau)-\Delta_{\tau}} \\
  &\beta(PP{}^{\mathrm{T}})\geq \frac{(1+c)\exp(-\gamma_{1}/\tau)-\Delta_{\tau}}{\exp(-\gamma_{k}/\tau)+\Delta_{\tau}} ~.
\end{align}
where
\begin{align}
\Delta_{\tau}=2\sqrt{k\frac{1}{T}(1+c)\log(2k/\delta)}
\end{align}
provided the number of feature points
\begin{align}
T\geq\frac{1}{9(1+c)}k\log(2k/\delta) ~.  
\end{align}
\end{thm}


Theorem \ref{thm:condition-number-P-under-fixed-tao} shows that when the number of features $T$ is large enough, the condition number $\beta(PP{}^{\mathrm{T}})$ is a random number concentrated around its expectation $(1+c)\frac{\exp(-\gamma_{1}/\tau)}{\exp(-\gamma_{k}/\tau)}$.
Since $\gamma_{1} \ll \gamma_{k}$, the numerator is much greater than the denominator when $\tau$ is fixed. Since our proof is based on Bernstein's Inequality, the upper bound is  tight. This forces $\beta(PP{}^{\mathrm{T}})$ to be a relatively large value. More specifically, the following corollary
shows that when $\gamma_{k}$ is linear to $\gamma_{1}$, $\beta(PP{}^{\mathrm{T}})$
is exponentially large in expectation. 
\begin{cor}
\label{def:cor}
When $\gamma_{k}\geq (M+1)\gamma_{1}$,
\begin{align}
\mathrm{E}\{\beta(PP{}^{\mathrm{T}})\} \geq
(1+c)[\exp(\frac{\gamma_{1}}{\tau})]^{M} \geq (1+c)(1+\frac{\gamma_{1}}{\tau})^{M}~.  
\end{align}
\end{cor}

Corollary \ref{def:cor} shows that when the actions in the video span across a
vast  range of dynamic (large M), the feature extractor with single $\tau$ tends
to have ill-conditioned feature matrices. A naive solution to this problem is to
increase $\tau$ to reduce the condition number in expection. However, this will
increase the variance $\Delta_\tau$ of $\beta(PP^T)$ because of a smaller number of features. In practice,  a large $\tau$  also increases the  difficulty in optical flow calculation and tracking. Hence, as will also be observed in
our experiments, choosing a good $\tau$ can be fairly difficult. Intuitively speaking, selecting $\tau$ is a trade-off between feature bias and variance.  A feature extractor with a large $\tau$ covers a long range of action signals but with less feature points hence generates features with small bias but large variance. Similarly, a feature extractor with a small $\tau$ will generate feature with large bias but small variance. 


\subsection{Condition Number of P under Multiple $\tau$}
\label{p3}

From Theorem \ref{thm:condition-number-P-under-fixed-tao}, to make $PP{}^{\mathrm{T}}$ well conditioned, we need $\tau$ as large as possible. However, when $\tau$ is too large, we cannot sample enough high quality feature points, the variance in $PP{}^{\mathrm{T}}$ will increase.
To address this problem, we propose to use MIFS, which incrementally enlarges the time skip $\tau$ , then stacks
all features under various $\tau_{i}$ to form a feature matrix. Hopefully, by
increasing $\tau$, we improve the condition number $\beta(PP{}^{\mathrm{T}})$
and by stacking, we sample enough features to reduce the variance.

Assuming we have features extracted from $\{\tau,2\tau,\cdots m\tau\}$. For $i\tau$ skip, the number of extracted features
$T_{i} = \left\lfloor 1/(i\tau)\right\rfloor $. The following theorem bounds
the condition number of MIFS.
\begin{thm}
\label{thm:condition-number-MSP} With probability at least $1-\delta$, the condition number of $PP{}^{\mathrm{T}}$
in the MIFS is bounded by
\begin{align}
\beta(PP{}^{\mathrm{T}})\leq  \frac{\sum_{i}\frac{T_{i}}{T}2(1+c)\exp(-\gamma_{1}/\tau_{i})+\Delta_{\tau}}{\sum_{i}\frac{T_{i}}{T}2\exp(-\gamma_{k}/\tau_{i})-\Delta_{\tau}}~.  
\end{align}
where
\begin{align}
\Delta_{\tau}\leq  2\sqrt{k\frac{1}{\sum_iT_i}(1+c)\log(2k/\delta)}~.
\end{align}
\end{thm}

Theorem \ref{thm:condition-number-MSP} shows that, in the MIFS, the expected condition number $\beta(PP{}^{\mathrm{T}})$ is roughly the weighted
average of condition numbers under various $\tau_{i}$. Since
$\tau_{i+1}>\tau_{i}$, the condition number under $\tau_{i+1}$ is smaller than
the one under $\tau_{i}$. Therefore, the condition number is reduced as we
expected. What's nicer is that the variance component $\Delta_{\tau}$ is
actually on order of $1/\sqrt{\sum_{i}T_{i}}$, which is also much smaller than a single $\tau$ scenario. In summary, we prove:
\begin{quote}
  The MIFS representation improves the learnability of differential
  feature extractor because it  reduces the expectation and variance of
  condition number $\beta(PP{}^{\mathrm{T}})$ simultaneously.
\end{quote}

==> ae.tex <==
\section{Additional Experiments}
\label{ae}
For completeness,  we conduct experiments on two additional benchmark datasets: UCF50 and Olympic Sports. The experimental settings are the same as in the paper. 
\paragraph{Datasets}
The UCF50 dataset \cite{reddy2013recognizing} has 50 action classes spanning over 6618 YouTube videos clips that can be split into 25 groups. The video clips in the same group are generally very similar in background. Leave-one-group-out cross-validation as recommended by \cite{reddy2013recognizing} is used and mean accuracy (mAcc) over all classes and all groups is reported. The Olympic Sports dataset \cite{niebles2010modeling} consists of 16 athletes practicing sports, represented by a total of 783 video clips. We use standard splits with 649 training clips and 134 test clips and report mAP as in \cite{niebles2010modeling} for comparison purposes. 

\paragraph{Results}

Table \ref{tab:scale_Pyramid_ap} lists the overall performances. Similar to what we have found in the HMDB51 dataset, the single-scale performance of UCF50 increase to $93.3\%$ MAcc from $93.0\%$ and decrease rapidly after that. Also, MIFS representations achieve much better performance than single-scale representations. In Table \ref{tab:state-of-art_ap}, we compare MIFS with $L=3$ performances to the state-of-the-arts. We can see that for UCF50, MIFS still enjoys a significant performance improvement over state-of-the-art methods, while for Olympic Sport datasets, the performance improvement is minimal due to inferior performance at $L=3$.   


\begin{table}
\centering
\caption{\label{tab:scale_Pyramid_ap}Comparison of different scale levels for MIFS.}
\begin{tabular}{|c | c |c |c |c | }
\hline
  & \multicolumn{2}{|c|}{UCF50  (MAcc$\%$) } & \multicolumn{2}{|c|}{ Olympics Sports (MAP$\%$)}  \\\hline
  L& Single-level & MIFS & Single-level & MIFS \\\hline 

 0 &   93.0 &                   & 89.8 &                 \\
 1 &   93.3 & 94.0              & 89.4 & \textbf{92.9}          \\
 2 &   92.2 & 94.1              & 88.1 & 91.7          \\
 3 &   89.7 & \textbf{94.4}     & 85.3 & 91.4 \\
 4 &   84.3 & \textbf{94.4}     & 85.0 & 90.3           \\
 5 &   76.7 & 94.3     & 82.3 & 91.3           \\
\hline
\end{tabular}

\end{table}



\begin{table}
\centering
\caption{\label{tab:state-of-art_ap}Comparison of our results to the state-of-the-arts.}
\begin{tabular}{|c c |c c|}
\hline
\multicolumn{2}{|c|}{UCF50 (MAcc. $\%$)} & \multicolumn{2}{|c|}{Olympics Sports (MAP $\%$)} \\
\hline
Shi \textit{et al.} \cite{shi2013sampling} 13 & 83.3 & Alexandros \textit{ et al.} \cite{iosifidis2014minimum} 14 & 78.6 \\
Sanath \textit{et al.} \cite{narayan2014cause} 14 & 89.4  & Jain \textit{et al.} \cite{jain2013better} 13  & 83.2 \\
Arridhana \textit{et al.} \cite{ciptadi2014movement} 14 & 90.0 &   Adrien \textit{et al.} \cite{gaidon2014activity} 14 & 85.5 \\
Oneata \textit{et al.} \cite{oneata2013action} 13 &90.0 & Oneata \textit{et al.} \cite{oneata2013action} 13 & 89.0 \\
 Wang \& Schmid \cite{wang2013action} 13  & 91.2 &  Wang \& Schmid \cite{wang2013action} 13  & 91.1 \\
\hline 
MIFS (L=3)  & \textbf{94.4} & MIFS (L = 3) &  \textbf{91.4}\\ 
\hline
\end{tabular}
\end{table}


==> review.tex <==


CVPR 2015
2015 IEEE Conference on Computer Vision and Pattern Recognition
Zhengzhong Lan 
Logout
Select Your Role: 	AuthorGo to Console
Manage
Submissions
View
Conference Status
Manage
Notes
View Author Feedback For Paper
Paper ID	1598
Title	Beyond Gaussian Pyramid: Multi-skip Feature Stacking for Action Recognition


 	Question	Response
1	Rebuttal	We thank the reviewers for their valuable feedback. We appreciate how they generally found our work interesting and novel, our analysis solid and our experiments thorough and convincing. The reviewers seem to share similar concerns, we will address them collectively.

Q: location(x,y,t) extension 
A: We include the location extension because we want to share the interesting observation that this extension is quite useful for action recognition. Although, it gives 2-5% improvement, it actually masks some performance gains MIFS can provide. Below is the performance w/o the extension. For HMDB51, without the extension, the improvement from L=0 to L=3 is 5.5% compared to 3% with it. Other datasets have similar patterns. R1 requested results of IDT with spatio-temporal pyramid, the results are worse than the location extension. We can add them in the final version. 
HMDB51 Hw2 UCF101 UCF50 Olympics
L=0: 57.9 64.7 86.2 91.1 89.9
L=3: 63.4 66.2 88.5 93.2 91.6

Q: Computational expense
A: In the common case (L=3), MIFS approximately doubles the computational cost of the original IDT. In the unlikely case of L=6, the feature extraction cost would be less than 2.6x the base cost. Spatial pyramid, with the recommended settings, is 8x as expensive as the basic BoF method. Gaussian pyramid adds computational costs similar to MIFS. Given how popular Spatial and Gaussian pyramids are, we feel some researchers will be willing to pay the cost to get the benefits. 
If computational cost is an issue, the method can be sped up by removing low-scale features. For example, removing L=0 (original videos) will significantly reduce cost but still give useful improvements as shown below. The bottom of the table shows the results of combining features from level 1 (every 2nd frame) and level 2 (every 3rd frame) but not L=0. As seen, we can still get better results with less cost. 
HMDB51 Hw2 UCF101 UCF50 Olympics Computational Cost
L=0: 62.1 67.0 87.3 93.0 89.8 1.0
L=2-0:63.9 67.6 88.5 93.8 91.9 0.75

Q: choosing the scale for different datasets and actions
A: As shown in the paper, different scale performance varies for different actions due to their speed range. We recommend L=3 based on extensive experiments and its physical meaning. For those who wish to find the optimal level, we recommend increasing L until the performance drops indicating the motion is too fast to be meaningful.

Q: Simplicity of our idea 
A: We readily acknowledge in the paper that the MIFS implementation is simple. Procedural simplicity should not be confused for trivial development. Many popular algorithms are simple ideas. For example, optical flow is just a derivative operation. We believe that the quality of an algorithm should be assessed by its mathematical properties and experimental results. We present the non-trivial theoretical underpinnings of MIFS, and experimentally show that it is useful. Although simple, MIFS improves IDT performance on all the datasets we have tested.

Q: Connection of differential operator and IDT
A: IDT has the appearance part and the motion part (optical flow). We model the optical flow, the displacement of two patches, as a differential operator. Fig. 3 shows the resulting feature matrices of IDT fits our theory. 

Q: Other issues
A: We thank R1 for suggesting the term ‘pooling’ and will use it in the final version. We apologize for the confusion of overloading of 'L' and will fix it. Regarding how MIFS changes with respect to trajectory length of IDT, we tested different IDT parameters including trajectory length, neighbor size, etc. for TRECVID MED competition, our experience is that MIFS is robust with respect to IDT parameters. We will use solid lines instead of dashed lines in Fig. 3.

©2007 Microsoft Corporation EULA  |  Terms of Use  |  Privacy Statement	 For Website related issues email CMT Support



CVPR 2015
2015 IEEE Conference on Computer Vision and Pattern Recognition
 	Reviews For Paper
Paper ID	1598
Title	Beyond Gaussian Pyramid: Multi-skip Feature Stacking for Action Recognition
Masked Reviewer ID:	Assigned_Reviewer_1
Review:	
Question	 
Paper and Review Summary. Briefly describe the contributions of the paper to computer vision. Include a concise, bulleted list of the paper's main strengths and a concise, bulleted list of the paper's main weaknesses. Please keep these brief. You will elaborate on the pros/cons in the subsequent text boxes below.	This paper proposes to enhance video representations for action recognition by combining features extracted at different time scales. A theoretical analysis shows that this improves the learnability of action models, as it improves the condition number of feature matrices. They significantly outperform the state of the art on five action recognition benchmarks (including the results in supplementary material), and outperform a single-scale baseline on TRECVID MED tasks.

Main strengths:
- solid theoretical analysis;
- convincing experiments.

Main weaknesses:
- small unclear contributions;
- overall lack of clarity;
- missing some baselines and references.
Paper Strengths. Please discuss the positive aspects of the paper. Be sure to comment on the paper's novelty, technical correctness, clarity and experimental evaluation. Notice that different papers may need different levels of evaluation: a theoretical paper may need no experiments, while a paper presenting a new approach to a known problem may require thorough comparisons to existing methods. Also, please make sure to justify your comments in great detail. For example, if you think the paper is novel, not only say so, but also explain in detail why you think this is the case.	The authors show that using multiple time "skips" improves the learnability of action models, thanks to a reduction of the expectation and variance of the condition number of the feature matrices. This theoretical analysis is solid, and is inline with the intuition that adding varied features improves the representation. The proofs are non-trivial, but seem correct.

The experiments are convincing too. The datasets chosen are challenging, realistic, and widely used in the community. The authors compare to the actual state of the art (and a bit more in fact as they consider an unpublished work [20]). Furthermore, they improve significantly over it --- even though a large part of this improvement is not due to their method, but they quantify this explicitly (comparison of [30] and L=0, lines 558-568). Note that the authors should include the results on UCF50 and Olympic Sports in the main text, instead of leaving it in the supplementary material, as they have almost a page of unused space (remember that references do not count).

Paper Weaknesses. Please discuss the negative aspects of the paper: lack of novelty or clarity, technical errors, insufficient experimental evaluation, etc. Please justify your comments in great detail. If you think the paper is not novel, explain why and give a reference to prior work. Keep in mind that novelty can take a number of forms; a paper may be novel in terms of the method, the theory, analysis for an existing problem, or the empirical evaluation. If you think there is an error in the paper, explain in detail why it is an error. If you think the experimental evaluation is insufficient, remember that theoretical results/ideas are essential to CVPR and that a theoretical paper need not have experiments. It is *not* okay to reject a paper because it did not outperform other existing algorithms, especially if the theory is novel and interesting. It is also not reasonable to ask for comparisons with unpublished papers and papers published after the CVPR deadline.	The method proposed here and the associated contributions are not clearly stated or described, including in the introduction. A partial description is given only in page 5 (lines 510-513): "The only difference between MIFS and other conventional methods is that instead of using feature points extracted from one time scale, we extract and stack all the raw feature points from different scales together before encoding.". Prior to that, only lines 124-125 give an idea of what this paper proposes: "gradually reducing the frame rate". Therefore, it seems that the only contribution is limited to a complex theoretical analysis of why extracting and combining features at different FPS is a good idea. This seems small, as this, indeed, is a straightforward way to address speed variations.

The text is also unclear due to the theoretical analysis formalizing feature extractors as temporal differential operators. This obfuscates the fact that MIFS consists in simply extracting features at different playback speeds, as explained above.

Furthermore, the connection between the features used here --- Improved Dense Trajectories (IDT) [33] --- and differential operators is not clear, and not explicitly made. In particular, [33] (and the other related CVPR'11 and IJCV'13 papers of Wang et al) do not describe or compute IDT from time differences as in Eq. 7. Consequently, it is unclear how the theoretical analysis is relevant for the features used in the experiments. If it is true, then this requires an explicit description of how to view IDT as differential operators (lines 301-304 are not sufficient).

The notion of "stacking" is also not described, and it seems that the features from different time scales are just pooled together (lines 510-513) instead of a concatenation like in spatio-temporal pyramids.

The notations are also confusing, especially regarding "L", at first the length of the video (line 303), and then the "level" of the MIFS without explanation (first use is line 561) or connection to the previously used \tau parameter.

Note also that the impressive performance improvements come mostly from a small modification of IDT [33] consisting in expanding local descriptors with (x,y,t) coordinates (line 508). Note that this is a standard trick of the trade in bag-of-visual-words-like models, and not a significant contribution here. By comparing lines 560-568 and Tables 1 & 2, we can see that this extension (results under L=0) improves by +2-5% w.r.t. [33], while using MIFS adds another +1-3% on top.

As a consequence of the previous remarks, it seems that the paper should include comparisons to more baselines in order to clarify the contributions. In particular, the paper should include experiments without the location trick (i.e. using only the same descriptors as [33]), with spatio-temporal pyramids (as in "Action and event recognition with Fisher Vectors on a Compact Feature Set", Oneata et al, ICCV'13), and with IDT extracted with different tracklet lengths (IDT use only 15 frames long trajectories, but can extract longer or shorter ones too).
Preliminary Rating: This rating indicates to the area chair, to other reviewers, and to the authors, your current opinion on the paper. Please use 'Borderline' only if the author rebuttal and/or discussion might sway you in either direction.	Borderline
Preliminary Evaluation. Please explain your current rating on the paper. This explanation may include how you weight the importance of the various strengths and weaknesses you described above in Q1-Q3. Note, after the rebuttal period, you will be asked to submit a response to the rebuttal and a final rating.	Although the theoretical analysis is nice and the experimental results are good, there is too much uncertainty on what is the precise contribution, what the method is actually doing, how it exactly relates to the theoretical analysis, and what is behind the performance gains. l think there is potential for a good paper, but it requires a significant amount of additional work.
Rebuttal Requests: Make a list of items you would like the authors to be sure to address in their rebuttal.	The authors need to clearly state what they propose, what is new, how their formalism and theoretical analysis relate to what they do in the experiments, and clearly explain where the performance gains come from via additional comparisons (cf. above).
Confidence. Select: "Very Confident" to stress that you are absolutely sure about your conclusions (e.g., you are an expert who works in the paper's area), "Confident" to stress that you are mostly sure about your conclusions (e.g., you are not an expert but can distinguish good work from bad work in that area), and "Not Confident" to stress that that you feel some doubt about your conclusions. In the latter case, please provide details in your Preliminary Evaluation response.	Very confident
Final Rating. Your choice should be justified in the Final Recommendation response.	Poster
Final Recommendation. Explain your final rating, taking into account the author's rebuttal and the discussion phase. Your explanation is essential for making informed acceptance decisions. It is also critical for deciding between posters and orals. Include suggestions for improvement where appropriate.	I recommend the paper as Poster.

After reading the other reviews and the rebuttal, I think that the authors answered most of our shared concerns (especially regarding the location extension and computational cost).

I still believe that they need to clarify their contributions a bit in the text, and make the link with the IDT features *explicitly*. I found the rebuttal on that latter point a bit light: sure, there are temporal derivatives involved somewhere in most motion features (as they are based on optical flow), but they give an explicit parametrization of the features in terms of differential operators, and this formalism needs to be instantiated with the features they use to explicit the link between the theory and the experiments.

All in all, I think this paper is first-and-foremost a collection of a couple of useful and high-performing tricks for action recognition. The theoretical sugar is nice, but it is not as convincing or insightful as the (extensive) experiments. Nevertheless, the sensible rebuttal makes me believe that the authors can improve the text to match the high quality of the experiments.

In summary, I do not think this paper is revolutionary, and that the maths are a bit misleading on that part, but the experiments, improvements over the state of the art, and simplicity of the method are, in my humble opinion, enough for an interesting CVPR poster.
Masked Reviewer ID:	Assigned_Reviewer_2
Review:	
Question	 
Paper and Review Summary. Briefly describe the contributions of the paper to computer vision. Include a concise, bulleted list of the paper's main strengths and a concise, bulleted list of the paper's main weaknesses. Please keep these brief. You will elaborate on the pros/cons in the subsequent text boxes below.	This paper proposed an approach called MIFS, which enhances current state-of-the-art features for action recognition by stacking features with different frequencies. The authors also proved that the feature matrices obtained by MIFS are stable with a small condition number. Better results were reported on several benchmarks, however at the cost of much more computational time.
Paper Strengths. Please discuss the positive aspects of the paper. Be sure to comment on the paper's novelty, technical correctness, clarity and experimental evaluation. Notice that different papers may need different levels of evaluation: a theoretical paper may need no experiments, while a paper presenting a new approach to a known problem may require thorough comparisons to existing methods. Also, please make sure to justify your comments in great detail. For example, if you think the paper is novel, not only say so, but also explain in detail why you think this is the case.	The idea of stacking features with different time skips is interesting. Results are also good.
Paper Weaknesses. Please discuss the negative aspects of the paper: lack of novelty or clarity, technical errors, insufficient experimental evaluation, etc. Please justify your comments in great detail. If you think the paper is not novel, explain why and give a reference to prior work. Keep in mind that novelty can take a number of forms; a paper may be novel in terms of the method, the theory, analysis for an existing problem, or the empirical evaluation. If you think there is an error in the paper, explain in detail why it is an error. If you think the experimental evaluation is insufficient, remember that theoretical results/ideas are essential to CVPR and that a theoretical paper need not have experiments. It is *not* okay to reject a paper because it did not outperform other existing algorithms, especially if the theory is novel and interesting. It is also not reasonable to ask for comparisons with unpublished papers and papers published after the CVPR deadline.	1.	Since MIFS requires much more computational efforts, it is difficult to apply MIFS to large scale datasets, for example, Deep Sports http://cs.stanford.edu/people/karpathy/deepvideo/

2.	In the experiment, it is very interesting to see that by adding three dimensional location features (L=0) , there will be 5%, 2.7% and 1.4% gains compared with Wang et al [33] on HMDB, Hollywood2 and UCF101 respectively. However, the performance gain of MIFS with L =3 compared with L=0 (3%, 1% and 1.8%) is not as significant as the aforementioned feature augmentation. To make a fair comparison with [33], I would like to see the performance of MIFS based on the original features [33] rather than the augmented ones. 

3.	Since the performance varies as L goes up across different benchmarks, how to choose the best L for a new dataset?

4.	I would like to see more discussions on the performance variations of different actions at different levels. 

5.	Minor: 1) The lines in Figure 3 are indistinguishable on a printed version. 2) L means level in Figure 2, whereas L means number of frames on line 303.
Preliminary Rating: This rating indicates to the area chair, to other reviewers, and to the authors, your current opinion on the paper. Please use 'Borderline' only if the author rebuttal and/or discussion might sway you in either direction.	Borderline
Preliminary Evaluation. Please explain your current rating on the paper. This explanation may include how you weight the importance of the various strengths and weaknesses you described above in Q1-Q3. Note, after the rebuttal period, you will be asked to submit a response to the rebuttal and a final rating.	The authors enhanced current state-of-the-art features by stacking features with different time skips, so that different action velocity can be incorporated in the MIFS feature representation. This feature representation outperforms state-of-the-art methods, but is less efficient. I would lean towards accept if the approach was more efficient.
Rebuttal Requests: Make a list of items you would like the authors to be sure to address in their rebuttal.	Please reply to the weak points given above.
Confidence. Select: "Very Confident" to stress that you are absolutely sure about your conclusions (e.g., you are an expert who works in the paper's area), "Confident" to stress that you are mostly sure about your conclusions (e.g., you are not an expert but can distinguish good work from bad work in that area), and "Not Confident" to stress that that you feel some doubt about your conclusions. In the latter case, please provide details in your Preliminary Evaluation response.	Confident
Final Rating. Your choice should be justified in the Final Recommendation response.	Poster
Final Recommendation. Explain your final rating, taking into account the author's rebuttal and the discussion phase. Your explanation is essential for making informed acceptance decisions. It is also critical for deciding between posters and orals. Include suggestions for improvement where appropriate.	This paper is a borderline case to me. I lean slightly towards acceptance because the approach is simple and the results are good.
Masked Reviewer ID:	Assigned_Reviewer_3
Review:	
Question	 
Paper and Review Summary. Briefly describe the contributions of the paper to computer vision. Include a concise, bulleted list of the paper's main strengths and a concise, bulleted list of the paper's main weaknesses. Please keep these brief. You will elaborate on the pros/cons in the subsequent text boxes below.	This paper describes a novel action representation based on Improved Dense Trajectory feature points extracted at different scales (typically 2-3). The proposed Multi-skIp Feature Stacking (MIFS) representation then filters (by a family of differential filters) and stacks the resulting multiple-scale features. Features are represented using several standard descriptors (HOG, HOF, ...) and encoded using Fisher Vectors. The experimental evaluation is complete, illustrative and convincing. Although this reviewer did not enter into the mathematical details, the formulation seems properly defined and derived.

The paper strengths of this paper are:
- The method exploits the fact that different actions need different scale ranges.
- The theoretical analysis on the MIFS learnability.
- A thorough experimental validation.

The paper weaknesses of this paper are:
- The high computational complexity of the method.
- For high scales the extracted features become less reliable.
Paper Strengths. Please discuss the positive aspects of the paper. Be sure to comment on the paper's novelty, technical correctness, clarity and experimental evaluation. Notice that different papers may need different levels of evaluation: a theoretical paper may need no experiments, while a paper presenting a new approach to a known problem may require thorough comparisons to existing methods. Also, please make sure to justify your comments in great detail. For example, if you think the paper is novel, not only say so, but also explain in detail why you think this is the case.	The paper strengths of this paper are:

- The method exploits the fact that different actions need different scale ranges.

- The complete demonstration that the MIFS representation improves the learnability of differential feature extractors.

- A thorough experimental validation, including having obtained excellent results in the TRECVID MED collections.
Paper Weaknesses. Please discuss the negative aspects of the paper: lack of novelty or clarity, technical errors, insufficient experimental evaluation, etc. Please justify your comments in great detail. If you think the paper is not novel, explain why and give a reference to prior work. Keep in mind that novelty can take a number of forms; a paper may be novel in terms of the method, the theory, analysis for an existing problem, or the empirical evaluation. If you think there is an error in the paper, explain in detail why it is an error. If you think the experimental evaluation is insufficient, remember that theoretical results/ideas are essential to CVPR and that a theoretical paper need not have experiments. It is *not* okay to reject a paper because it did not outperform other existing algorithms, especially if the theory is novel and interesting. It is also not reasonable to ask for comparisons with unpublished papers and papers published after the CVPR deadline.	The paper weaknesses of this paper are:

- The high computational complexity of the method. This is mainly due to the fact that the bottleneck of the method is the extraction of the dense trajectory features. It would be interesting then to compare the complexity of the proposed representation (dimensionality, learning time) w.r.t. existing alternatives like [20, 33] and, in addition, to propose ways for reducing the training time.

- As already commented by the authors, for high scales the extracted features become less reliable. Therefore, it is not worth to consider more than 4 scales, although the approach already outperforms SoA with less than 3 scales.

- Since a deep analysis of the best- and worst-performing action events for the datasets can be found at the supplementary file, it would be interesting to include a reasoned paragraph describing (roughly) which types of events are better/worse recognised by the MIFS representation, and why (role of the event complexity, background clutter, different action speeds, ...).
Preliminary Rating: This rating indicates to the area chair, to other reviewers, and to the authors, your current opinion on the paper. Please use 'Borderline' only if the author rebuttal and/or discussion might sway you in either direction.	Accept
Preliminary Evaluation. Please explain your current rating on the paper. This explanation may include how you weight the importance of the various strengths and weaknesses you described above in Q1-Q3. Note, after the rebuttal period, you will be asked to submit a response to the rebuttal and a final rating.	The paper presents a multi-scale representation for action recognition. The theoretical analysis and the experimental validation are convincing. In general, the approach is interesting and the resulting multi-scale descriptor clearly outperforms current state-of-the-art. For example, the results obtained for the TRECVID MED task is of merit.
Rebuttal Requests: Make a list of items you would like the authors to be sure to address in their rebuttal.	No particular requests are demanded at the rebuttal.
Confidence. Select: "Very Confident" to stress that you are absolutely sure about your conclusions (e.g., you are an expert who works in the paper's area), "Confident" to stress that you are mostly sure about your conclusions (e.g., you are not an expert but can distinguish good work from bad work in that area), and "Not Confident" to stress that that you feel some doubt about your conclusions. In the latter case, please provide details in your Preliminary Evaluation response.	Very confident
Final Rating. Your choice should be justified in the Final Recommendation response.	Poster
Final Recommendation. Explain your final rating, taking into account the author's rebuttal and the discussion phase. Your explanation is essential for making informed acceptance decisions. It is also critical for deciding between posters and orals. Include suggestions for improvement where appropriate.	The paper presents a multi-scale representation for action recognition. The theoretical analysis and the experimental validation are convincing. In general, the approach is interesting and the resulting multi-scale descriptor clearly outperforms current state-of-the-art. For example, the results obtained for the TRECVID MED task is of merit.


 
